mmFUSION: Multimodal Fusion for 3D Objects Detection

Multi-sensor fusion is essential for accurate 3D object detection in self-driving systems. Camera and LiDAR are the most commonly used sensors, and usually, their fusion happens at the early or late stages of 3D detectors with the help of regions of interest (RoIs). On the other hand, fusion at the intermediate level is more adaptive because it does not need RoIs from modalities but is complex as the features of both modalities are presented from different points of view. In this paper, we propose a new intermediate-level multi-modal fusion (mmFUSION) approach to overcome these challenges. First, the mmFUSION uses separate encoders for each modality to compute features at a desired lower space volume. Second, these features are fused through cross-modality and multi-modality attention mechanisms proposed in mmFUSION. The mmFUSION framework preserves multi-modal information and learns to complement modalities' deficiencies through attention weights. The strong multi-modal features from the mmFUSION framework are fed to a simple 3D detection head for 3D predictions. We evaluate mmFUSION on the KITTI and NuScenes dataset where it performs better than available early, intermediate, late, and even two-stage based fusion schemes. The code with the mmdetection3D project plugin will be publicly available soon.

==> backups.tex <==

\begin{table*}[t!]
    \centering
    \caption{Comparisons of different multi-modality fusion methods with our mmFUSION on the NuScenes \textit{val set} and \textit{test set}}
    \begin{tabular}{lccccccc}
         \hline
         Method & Fusion Scheme& NDS(val) & mAP(val) & NDS(test & mAP(test) & MACs(G) & Latency(ms) \\
        \hline
         
         FUTR3D\cite{chen2023futr3d}&feats&68.30&64.3&--&--&1069&321.4\\
         FusionPainting\cite{xu2021fusionpainting}&early&70.70&66.50&71.6&68.1&--&--\\
         AutoAlign\cite{chen2022autoalign}&late&71.10&66.60&--&--&--&--\\
         PointPainting\cite{vora2020pointpainting}&early&69.60&65.80&--&--&370.0&185.8\\
         PointAugmenting\cite{wang2021pointaugmenting}&early+feats&--&--&71.0&66.8&408.5&234.4\\ 
         MVP\cite{yin2021multimodal}&early&70.00&66.10&70.5&66.4&371.7&187.1\\
         TransFusion\cite{bai2022transfusion}&feats&71.30&67.50&71.6&68.9&485.8&156.6\\
         BEVFusion\cite{liu2022bevfusion}&feats&71.40&68.50&72.9&70.2&253.2&119.2\\
         mmFUSION\textbf{(ours)}&feats&69.75*&64.67*&**&**&**&**\\ 
         \hline
         
    \end{tabular}
    \textit{* means this value will be updated after getting updated results} \\
    \label{tab:NuScenes_val_and_test}
\end{table*}










\begin{table*}[t!]
    \centering
    \caption{Comparison of mmFUSION with recent methods of early, late, and intermediate (feats.) level fusion on nuscenes \textit{val set}. We compare overall and at per class level as well.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llcccccccccccc}
         \hline
         Method & Backbone (2D+3D)&\textbf{NDS(\%} & \textbf{mAP(\%)} & Car & Truck&C.V& Bus& Trailer & Barrier &Motor.& Bike&Ped.& T.C.\\
        \hline
        FusionPainting\cite{xu2021fusionpainting}& HTCNet+SECOND&67.41&62.15&83.98&59.97&22.90&71.13&41.53&63.29&66.85&54.35&82.86&74.66\\
         FUTR3D\cite{chen2023futr3d}& R101+SECOND&68.30&64.50&86.30&61.50&26.00&71.90&42.10&64.40&73.60&63.30&82.60&70.10\\
         VFF\cite{li2022voxel}&R50+CenterPoint&68.70&63.40&86.40&60.10&23.80&71.70&38.80&68.00&71.50&52.20&86.20&75.80\\
         
         mmFUSION \textbf{(ours)} &R50+SECOND&\textbf{69.75}&\textbf{65.43}&\textbf{87.60}&60.79&\textbf{28.50}&\textbf{72.62}&40.62&67.24&\textbf{74.02}&\textbf{65.17}&85.24&72.46\\
         
         \hline
    \end{tabular}
    }
    \label{tab:NuScenes_val_on_class_level}
\end{table*}



\begin{table*}[t!]
    \centering
    \caption{Comparison of mmFUSION with UVTR \cite{li2022unifying} on nuscenes \textit{val set}}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llccccccc}
         \hline
         Method & Backbone(img+pts)& \textbf{NDS(\%} & \textbf{mAP(\%)} & mATE \downarrow& mASE \downarrow& mAOE \downarrow & mAVE \downarrow & mAAE \downarrow \\
        \hline
         %UVTR\cite{li2022unifying}&R50+SECOND&65.60&60.10&--&--&--&--&--\\
         %VFF\cite{li2022voxel}&R50+CenterPoint&68.70&63.40&--&--&--&--&--\\

         UVTR\cite{li2022unifying}&R101+SECOND&70.20&65.40&0.333&0.258&0.270&0.216&0.176\\
         mmFUSION \textbf{(ours)} &R50+SECOND&69.75&\textbf{65.43}&\textbf{0.327}&\textbf{0.256}&\textbf{0.268}&0.219&\textbf{0.170}\\
         %\hline
         %FUTR3D \cite{chen2023futr3d}&R101+SECOND&68.30&64.50&--&--&--&--&--\\
         
         %mmFUSION \textbf{(ours)} &R101+SECOND&--&--&--&--&--&--&--\\ 
         
         \hline
    \end{tabular}
    }
    
    \label{tab:NuScenes_val_with_dff_bbs}
\end{table*}


